ShearLab 3D: Faithful Digital Shearlet Transforms based on Compactly Supported Shearlets

Wavelets and their associated transforms are highly efficient when approximating and analyzing one-dimensional signals. However, multivariate signals such as images or videos typically exhibit curvilinear singularities, which wavelets are provably deficient of sparsely approximating and also of analyzing in the sense of, for instance, detecting their direction. Shearlets are a directional representation system extending the wavelet framework, which overcomes those deficiencies. Similar to wavelets, shearlets allow a faithful implementation and fast associated transforms. In this paper, we will introduce a comprehensive carefully documented software package coined ShearLab 3D (www.ShearLab.org) and discuss its algorithmic details. This package provides MATLAB code for a novel faithful algorithmic realization of the 2D and 3D shearlet transform (and their inverses) associated with compactly supported universal shearlet systems incorporating the option of using CUDA. We will present extensive numerical experiments in 2D and 3D concerning denoising, inpainting, and feature extraction, comparing the performance of ShearLab 3D with similar transform-based algorithms such as curvelets, contourlets, or surfacelets. In the spirit of reproducible reseaerch, all scripts are accessible on www.ShearLab.org.

==> tex2bib <==
#! /usr/local/bin/perl 

$Script = 'tex2bib'; 
$Version=0.97;  # 22 Feb 2006 10:50:35
$Author='Michael Friendly (friendly@yorku.ca)';

# Copyright (c) 1997 Michael Friendly
#
# License:
#  This is free software subject to copyright, released according to the
#  BSD style license.  It may be freely used, modified and distributed.
#  See: http://www.ctan.org/tex-archive/help/Catalogue/licenses.bsd.html
#  for details and further information.

# tex2bib
#   Input a TeX document containing \bibitems, translate these
#   to BibTeX format
#
# Usage:
#		tex2bib [-k][-i infile] [-o outfile]
#		-k:  regenerate keys
#		if infile not given, reads from stdin
#		if outfile not given, prints to stdout

# The entire tex document is scanned for \bibitems, ending when
# the string '\end{thebibliography}' is read.

# Assumes that bibitems are formatted as follows:
#  -- {key}author(s), (date) at the beginning
#  -- titles of books or names of journals: {\em title}
#  -- article titles: 	after date, `` '' quotes optional
#  -- volume, pages: 	{\it vol}, nnn-nnn.
#  -- publisher/address:    address:publisher
#
#  All text in the bibitem which cannot be parsed is included
#  in a note = { } field
#
# Changes
#  0.96 1998/06/22  Allow \bibitem keys to contain [\w:-]
#  0.97 2006/02/21  Added BSD license
#################################################################
# Examples of a book, article, inproceedings:

#\bibitem{Bertin83}Bertin, J. (1983),
#        {\em Semiology of Graphics} (trans. W. Berg).  Madison, WI:
#        University of Wisconsin Press.
#
#\bibitem{Bickel75}Bickel, P. J., Hammel, J. W. and O'Connell, J. W.
#        (1975).
#        Sex bias in graduate admissions: data from Berkeley.  {\em
#        Science}, {\it 187}, 398-403.
#
#\bibitem{Farebrother87}Farebrother, R. W. (1987),
#        ``Mechanical representations of the ${L}_1$ and ${L}_2$ estimation
#        problems'', In Y. Dodge (ed.)  {\em Statistical data analysis
#        based on the L1 norm and related methods}, Amsterdam:
#        North-Holland., 455-464.


# These are output as:

#@Book{  Bertin:83,
#    author      = {J. Bertin},
#    year        = 1983,
#    title       = {Semiology of Graphics},
#    publisher   = {University of Wisconsin Press},
#    address     = {Madison, WI},
#    note        = {(trans. W. Berg).}
#}
#@Article{       Bickel:75,
#    author      = {Bickel, P. J. and Hammel, J. W. and O'Connell, J. W.},
#    year        = 1975,
#    title       = {Sex Bias in Graduate Admissions: Data from Berkeley},
#    journal     = {Science},
#    volume      = 187,
#    pages       = {398-403}
#}
#@InCollection{  Farebrother:87,
#    author      = {R. W. Farebrother},
#    year        = 1987,
#    title       = {Mechanical Representations of the ${L}_1$ and ${L}_2$ Estimation Problems},
#    booktitle   = {Statistical Data Analysis Based on the L1 Norm and Related Methods},
#    editor      = {Y. Dodge},
#    publisher   = {North-Holland},
#    address     = {Amsterdam},
#    pages       = {455-464}

# Text in a bibitem is removed from the bibitem as it is assigned to
# bibtex fields.  Any text remaining is assigned to a note={  } field
# at the end.  Since the parsing is heuristic, some manual fixup work
# can be expected at the end.

#################################################################

require 'getopt.pl' ;

    Getopt("oikdrt:");             # ARGV now contains [inputfile] and
                                #   $opt_o, $opt_i might be set.
	
	$default_type = $opt_t || 'Article';
	
    open(STDIN, "<$opt_i") or die "-i $opt_i: can't open.\n" if $opt_i ;
    open(STDOUT, ">$opt_o") or die "-o $opt_o: can't create.\n" if $opt_o ;

#######################  Process input files  ####################
$bibs=0;
while (<>)
{
	/^\s*\\end\{thebibliography/ && last;
	if (/\\bibitem\s*\{([\w\d:-]+)\}/) {
		$bibs++;
		$key = $1;
#		print STDERR "$bibs key: $key\n";
	}
	# skip if we're still reading tex text (no bibitems encountered)
	next unless $bibs;
	chomp;
	s/^\s*/ /;
	$lines .= $_;
}

# All lines containing \bibitems have been read into the $lines string.
# Now, split into separate items

@items = split(/\\bibitem\s*/, $lines);
print STDERR "items has ", scalar(@items), " items\n";

@months = qw(january february march april may jun july august september
	october november december);
$month_pat = join('|', @months);

foreach (@months) {
	$month_abbrv{$_} = substr($_, 0,3);
}
	
$ordinal = 'first|second|third|fourth|1st\.?|2nd\.?|3rd\.?|4th\.?';

# title words to ignore for casing;
foreach ( qw(a about an and by for from in of on the to von with) ) {
	$ignore_case{$_} = 1;
}

$outitems =0;
%keys_seen = {};

foreach $i (0..$#items) {
	undef $title;
	undef $pages;
	undef $journal;
	undef $volume;
	undef $number;
	undef $booktitle;
	undef $editor;
	undef $edition;
	undef $month;
	undef $publisher;
	undef $address;
	undef $chapter;
	undef $rest;
	
	print "$items[$i]\n" if $opt_d;
	# assume each entry starts with
	#	{key}Author, F.I. etc (date[a-z]?)
#	$items[$i] =~ /^\{([^}]+)\}([^\(]*)\((\d{4})[a-z]?\)[,.]?\s*/;
#	($key, $authors, $date) = ($1, $2, $3);
	$items[$i] =~ /^\{([^}]+)\}\s*/;
	$key = $1;
#	print  "key: $key\n";
	$rest = $';
		
	$rest =~ /\((\d{4})[a-z]?\)[,.]?\s*/ &&
		do {
			$authors = $`;
			$date = $1;
			$rest = $';
		};

	unless (defined($key)) {
		print STDERR "Skipping: $authors, $date in \n$items[$i]\n";
		next;
	}
		

	$rest =~ s/^[.,]?\s+//;
	$rest =~ s/\s+$//;

#	print "key: $key\n";
#	$key =~ m/(['A-Za-z]+)([^:]*)/ &&
#		do { $key = "$1:$2"; };
#	print "key: $key\n";
			
	&parse_authors;

	$orig_key = $key;
	$key = &generate_key if $opt_k or $keys_seen{$key};
	
	# if the $key has already been seen, make a new, unique one
	if ($keys_seen{$key}) {
		foreach $suffix (('b'..'z')) {
			$try = $key . $suffix;
#			print STDERR "Seen $key ... trying $try\n";
			unless ($keys_seen{$try}) {$key = $try; last; };
		}
		print STDERR "New unique key generated: $key (was $orig_key)\n"
			unless $key eq $orig_key;
	}
	$keys_seen{$key}++;
	
	# assume it's an article at first
	$type = '@' . $default_type;

	if ($rest =~ /^\{\\em\s+/) {
	#tech report or book
		$type = '@Book';
		$rest =~ m/^\{\\em\s+(['\w ,?:]+)\}[., ]*/;
		$title = $1;
		$rest = $';
		&parse_edition;
		&parse_publish;

		$rest =~ m/\sreport(s?)[,]?\s*/i &&
			do {
				$type ='@TechReport';
				$rest = $` . $';
				&parse_report_number;
			};
	}

	else {
		#does it begin with quoted title?
		if ($rest =~ /^``/){
			$rest =~ m/^``([^`]+)''[., ]*/;
			$title = $1;
			$rest = $';
		}
		else {
			$rest =~ m#^(['\{\}\w\d,\(\)\\ :\?/-]+)[. ]*#;
			$title = $1;
			$rest = $';
		}
		$rest =~ s/^[,\s]+//;
		
		if ($rest =~ /^\{\\em\s+/) {
			$rest =~ m/^\{\\em\s+([\w\\& ,'-?]+)\}[., ]*/;
			$journal = $1;
			$rest = $';
		}
		# parse {\it volume (number)}
		&parse_volume;
			
		$rest =~ m/,?\s*(\d{1,4}--?\d{1,4})[.,]?\s*/ && 
			do {
			$pages = $1;
			$rest = $`. $';
			$pages =~ s/(\d)-(\d)/$1--$2/;
			};

		$rest =~ m/\(($month_pat)\)/i &&
			do {
				($month = $1) =~ tr/A-Z/a-z/;
				$month = $month_abbrv{$month};
				$rest = $` . $';
			};
			
		$rest =~ m/(technical|tech\.)\s+report[,.]?/i &&
			do {
				$type ='@TechReport';
				$rest = $` . $';
				&parse_report_number;
			};
		
		$rest =~ m/^In\s+/i &&
			do {
				$rest = $';
				$type ='@InCollection';  # maybe, proceedings
				$rest =~ m/\{\\em\s+([\w ,':!?]+)\}[., ]*/ &&
					do {
					$booktitle = $1;
					$rest = $` . $';
					$type = '@InProceedings' if $booktitle =~ m/proceedings/i;
					};
				$rest =~ m/([\w., ]+)\s+\(eds?\.\)[,.]?\s*/i &&
					do {
					$editor = $1;
					$rest = $` . $';
					};
				$rest =~ m/Chapter\s+(\d+)[.,]?\s*/i &&
					do {
					$chapter = $1;
					$rest = $` . $';
					};
				
				&parse_edition;
				&parse_publish;
			};

		$rest =~ m/proceedings/i &&
			do {
				$type = '@InProceedings';
#	print "$items[$i]\n";
			};
	}

	$rest =~ s/^\s+//;
	$rest =~ s/$date([,]?)//;
	
	$title = &case_title($title);
	$booktitle = &case_title($booktitle) if $booktitle;
	
	print "$type\{$key";
	print ",\n    author\t= {$authors}";
	print ",\n    year\t= $date";
	print ",\n    title\t= {$title}" if $title;
	print ",\n    booktitle\t= {$booktitle}" if $booktitle;
	print ",\n    edition\t= {$edition}" if $edition;
	print ",\n    editor\t= {$editor}" if $editor;
	print ",\n    publisher\t= {$publisher}" if $publisher;
	print ",\n    address\t= {$address}" if $address;
	print ",\n    journal\t= {$journal}" if $journal;
	print ",\n    volume\t= $volume" if $volume;
	print ",\n    month\t= $month" if $month;
	print ",\n    number\t= $number" if $number;
	print ",\n    pages\t= {$pages}" if $pages;
	print ",\n    chapter\t= {$chapter}" if $chapter;
	print ",\n    note\t= {$rest}" if $rest;
	print "\n\}\n";
	$outitems++;	
}
print STDERR "$outitems items processed\n";
exit;

########################### subroutines #############################

# separate multiple authors with 'and'
sub parse_authors {
	# fix authors field
	$authors =~ s/\s+$//;
	$authors =~ s/\\&/and/;
	$authors =~ s/([A-Z])\.([A-Z])\./$1. $2./g;
	$authors =~ s/ ([A-Z])\.,\s+(?!Jr.)/ $1. and /g;
	$authors =~ s/ and and / and /;
#	$authors =~ s/Friendly, M./Friendly, Michael/;
	$authors =~ s/M. Friendly/Friendly, M./;
	local($commas) = ($authors =~ tr/,/,/);
	if ($opt_r && $commas == 1) {
		@auth = split(/, /, $authors);
		$authors = join(' ',reverse(@auth));
	}

}

# extract last names of authors into @auth array
sub split_authors {
	@auth = split(/ and /, $authors);
	@auth =~ grep(s/, .*$//g,@auth);          # strip trailing initials
	@auth =~ grep(s/^([A-Z]\.\s*)+//g,@auth);
#	@auth =~ grep(s/^[a-z ]+//,@auth);        # strip any name prefixes

	foreach  $i (0..$#auth) {
		@n = split(/ /, $auth[$i]);
		$auth[$i] = pop(@n);               # strip anything before lastname
		$auth[$i] =~ s/[^\w]//g;           # remove non-word chars 		
	}
		
#	print STDERR "Authors: $authors --> ", 
		join('|',@auth),"\n"    if scalar(@auth) > 1;
		
}

sub parse_volume {
	$rest =~ m/,?\s*\{\\it\s+([A-Za-z \d()]+)\s*\}[.,]?/ &&
		do {
		$volume = $1;
		$rest = $`. $';
		$volume =~ m/\(([ \w]+)\)/ &&
			do {
				$volume = $`;
				$number = $1;
			};
		$volume = "{$volume}" unless $volume =~ m/^\d*$/;
		$number = "\{$number\}" unless $number =~ m/^\d*$/;
		};
			
}

# find publisher and address in book/inproceedings items
#	assume the format is address:publisher
sub parse_publish {
	local($before, $after);
	$rest =~ m#:\s*([\w-\\/& ]+)[.]?# &&
		do {
			$publisher = $1;
			($before, $after) = ($`, $');
			$before =~ m/([\w, ]+)$/ &&
				do {
				$address = $1;
				$before = $`;
				$address =~ s/^\s+//;
				};
			$rest = $before . $after;
		};
}

sub parse_report_number {
	$rest =~ m/\s*(no\.|number)\s+(\d+)[,.]?\s*/i &&
		do {
		$number = $2;
		$rest = $` . $';
		}
}

sub parse_edition {
	$rest =~ m/\(?($ordinal).*(edition|ed\.)\)?\.?\s*/i &&
		do {
		$edition = $1;
		$rest = $` . $';
		}
}

# Initial-caps for all non-ignored words
sub case_title {
	local($t) = @_;
	local(@words) = split(/\s+/, $t);
	local($w) =0;
	local($colon);
	foreach (@words) {
		$w++;
		next if /^[A-Z]/;
		unless ($colon) {next if $ignore_case{$_}};		
		s/^([a-z])/\u$1/;
		$colon = tr/:/:/;
	}
	join(' ', @words);
}

sub generate_key {
	local($yr, $key);
	($yr = $date) =~ s/^1\d//;
	&split_authors;	
	if (scalar(@auth) < 3) {
		$key = join('', @auth, ':', $yr);
	}
	else {
		$key = join('', $auth[0], '-etal:', $yr);
	}
#	print STDERR "New key: $key (", join('|', @auth), ": $date)\n";
	$key;
}

